Adversarial Data Collection: Human-Collaborative Perturbations for Efficient and Robust Robotic Imitation Learning

The pursuit of data efficiency, where quality outweighs quantity, has emerged as a cornerstone in robotic manipulation, especially given the high costs associated with real-world data collection. We propose that maximizing the informational density of individual demonstrations can dramatically reduce reliance on large-scale datasets while improving task performance. To this end, we introduce Adversarial Data Collection, a Human-in-the-Loop (HiL) framework that redefines robotic data acquisition through real-time, bidirectional human-environment interactions. Unlike conventional pipelines that passively record static demonstrations, ADC adopts a collaborative perturbation paradigm: during a single episode, an adversarial operator dynamically alters object states, environmental conditions, and linguistic commands, while the tele-operator adaptively adjusts actions to overcome these evolving challenges. This process compresses diverse failure-recovery behaviors, compositional task variations, and environmental perturbations into minimal demonstrations. Our experiments demonstrate that ADC-trained models achieve superior compositional generalization to unseen task instructions, enhanced robustness to perceptual perturbations, and emergent error recovery capabilities. Strikingly, models trained with merely 20% of the demonstration volume collected through ADC significantly outperform traditional approaches using full datasets. These advances bridge the gap between data-centric learning paradigms and practical robotic deployment, demonstrating that strategic data acquisition, not merely post-hoc processing, is critical for scalable, real-world robot learning. Additionally, we are curating a large-scale ADC-Robotics dataset comprising real-world manipulation tasks with adversarial perturbations. This benchmark will be open-sourced to facilitate advancements in robotic imitation learning.

==> 1-Data_collection_fengsiyuan.tex <==


 
% 一、	发明名称及技术领域
% 发明名称：对抗式端到端机器人数据采集。
% 本发明适用于通用机器人产品的端到端模仿学习任务数据采集。
% 二、	背景技术
% 现有机器人端到端模仿学习任务采集缺乏系统性的理论支持。已有的知名工作如清华交叉信息研究院高阳老师组提出的Data Scaling Laws in Imitation Learning for Robotic Manipulation，梳理了模型性能随着数据集大小、模型大小和计算资源大小的关系。主要发现有：
% 1. 数据规模化定律的存在，即泛化能力与数据量呈幂律关系。
% 2. 多样性的重要性超过演示次数，环境和物体的多样性是关键。
% 3. 高效的数据收集策略，少量演示但多样环境即可实现高成功率。
% 这些重要发现指出了数据演示方案从环境和物体多样性上对于机器人端到端学习的重要意义。然而，现有的理论框架仍缺乏重要的一个环节，即数据采集动作方案对于机器人学习的影响、以及何种动作方案可以最大化采集效率，仍然缺乏理论支持。
% 我们提出的对抗式机器人数据采集首次在数据采集动作上提出了一个系统性的解决方案。经过实验，在主要机器人操作任务上，对抗式机器人数据采集可以以10%到20%的数据采集代价达到原先数据采集的效果；同时，对抗式机器人数据采集显著提升了对场景的泛化能力。
% 三、	技术方案的详细阐述
% 对抗式数据采集的核心是在机器人工作过程中，在外界环境引入干扰系统，执行不同类型的干扰，使得机器人难以以简单固定的动作路径完成任务。同时，机器人的所有策略都是在主动克服干扰、恢复被破坏的外界状态到指令状态，因此机器人的所有策略优化方向都是导向完成任务目标，所以不存在模仿学习过程中学习到不良策略的趋势。可以说，这样的数据采集策略大幅度提升了状态空间探索效率、提高了对外界环境变化时的泛化能力。
% 原先的端到端模仿系统如下图所示，是首先使用采集系统采集机器人数据，然后使用这些机器人数据进行训练。得到训练的模型后，模型在机器人上进行实机部署推理，指挥机器人进行工作。我们提出了对抗式采集，即引入干扰系统，在采集时对采集系统进行各类扰动，从而得到非常高质量的数据。通过这样的数据训练，我们只需要较原先10%的数据就可以获得一样的效果，同时还可以系统性涌现出被操作物体跟随、语言指令跟随、主动避障、主动柔顺控制等能力。其中，干扰系统可以由不同的系统实现，如使用仿真工具、真实场景中使用场景自动化道具、或者使用人工进行。具体的扰动方式描述如下。
% 1. 抓取、转移与放置（Pick, Place and Transfer）
% (1)	位置扰动：被抓取物体在空间位置上以符合随机分布（如高斯分布）的初始位置放置。在机器人执行抓取时，被抓取物体执行匹配机器人抓取速度的逃逸策略。逃逸策略包括突然改变运动方向，和在机器人可抓取范围内爆发式移动（如干扰系统需要在一秒内完成干扰）。采集系统需要实时做出响应、尽力在最短时间内抓到物体。
% (2)	抓取姿态扰动：当被抓取物体进入机器人末端执行器抓取范围中时，干扰系统进行爆发式干扰，在几百毫秒内使得被抓取物体姿态产生较大变化，使得机器人无法以最优抓取姿态控制物体。采集系统需要重新调整姿态来重新抓取，直到采集系统可以以最优姿态抓住物体。
% (3)	放置位置干扰：放置位置执行类似上文中位置扰动的策略。放置位置常常与具体语言指令相关，因此在下文与语言指令建立关联中进行详细描述。
% 2. 灵巧操作（Dexterous Manipulation）
% 如涉及到了柔性物体的旋转、堆叠、翻转等复杂、连续性任务，是业界的难题。其核心原因是这类任务涉及的状态空间大、难以有限的状态来表征事物状态。因此，对于灵巧操作任务，干扰系统不断在不同的时刻破坏采集系统已经达成的效果，尽可能多样的、复杂的破坏任务，让机器人从不同的状态起始点都可以达成目标效果。
% 实施例1：整理桌面。给定桌面的整理参考构型，以任意混乱初始状态开始，机器人开始执行整理策略。每一步的整理策略可以大致看为一个抓取、转移与放置任务。在每一步中，干扰系统使用上一节中位置干扰指令。
% 实施例2：叠衣服。给定任务混乱的初始衣物，机器人开始执行整理策略。整理过程中，干扰系统不断执行状态破坏，如将折叠一半的衣服翻开一个角，将伸展的衣物堆出多余皱褶等。
% 实施例3：擦拭不规则液体污渍。干扰系统给定不规则形状液体，在机器人执行清理任务的时候在机器人执行的任意阶段，在机器人可操作空间内的任意位置、泼洒任意大小的污渍。机器人以最小的移动轨迹、实时根据最新的污渍形态进行擦拭。
% 3. 与语言指令建立关联
% 语言指令是机器人端到端操作的另一大核心模块。由于神经网络特别擅长从任何线索中挖掘关联，且语言模块的信息量大大低于视觉，因此在机器人端到端训练时，尤其需要有效提升机器人遵循语言输入的能力。对抗式采集同样有助于克服模型容易从视觉信号进行学习、有效提升机器人理解并遵循语言指令的能力。具体方法是：
% (1)	随时打断：在采集系统执行指令时，对抗系统可以随时用新指令打断；采集系统需要立刻予以响应，在保证安全的条件下立刻停止执行当前任务，并去执行对抗系统发出的指令。
% (2)	屏蔽视觉线索：在完全相同的场景设置下，设置多种不同的任务类型，任务类型仅靠语言可以分辨。对抗系统在采集系统工作时，根据随时打断的原则随时切换任务类型，采集系统根据干扰系统指令去执行相应的任务。
% (3)	空指令、无关指令对抗：语言指令可能存在错误，也可能有停止工作的指令。在收到与当前场景无关、无法执行的指令，或者指令为空的时候，采集系统在保证安全的条件下立刻停止工作，直到可以执行的指令出现。
% (4)  更换指令：更换指令
% 4. 接触与力控类任务与主动避障安全能力
% 触觉传感器、关节力矩传感器、末端六维力传感器等力传感器信号对于涉及到柔顺控制的任务非常重要，尤其对于带有紧密配合等视觉难以判断的任务，机器人需要依靠力传感器执行。对于涉及到柔顺控制任务和主动安全的任务，对抗系统要求从环境中对采集系统进行涉及到显著力变化、带有碰撞风险的干扰。采集系统必须立刻响应外界变化，以合适大小的力执行任务、且需要保证安全。
% 实施例1：擦拭类清洁任务、打磨等接触任务。如擦拭桌面，采集系统的任务是以合适的力来接触桌面并执行擦拭，需要配置快速可动桌面；或者可以快速调整的机器人基座供干扰系统执行干扰。干扰系统在擦拭过程中突然变动桌面高度/机器人高度，反复造成机器人擦拭的力突变，机器人立刻根据力的方向调整接触位置，来恢复合适的接触力。
% 实施例2：紧密配合时装配和拆卸。对于带有紧密配合的装配和拆卸任务，干扰系统不断以视觉难以捕捉的幅度（如小于10mm）对被装配物体执行爆发性扰动，导致采集系统无法立刻完成任务。采集系统需要即刻进行反应，轻微调整接触力大小，来完成任务执行。
% 实施例3：通用主动避障干扰。对于大部分的机器人任务执行，操纵物体时需要精巧的避开障碍物，如从料盘中取料时需要避免碰撞其他物料和料盘、从货架上取料需要避免碰撞其他物料和货架，底盘运动时需要避开地面的障碍物。干扰系统需要进行突然接近机械臂或机器人本体的非操作物体，如料盘和货架，导致它们过分接近甚至直接与机械臂发生碰撞。采集系统应当实时做出反应，尽量远离障碍物、保持合适距离。
% 四、	核心发明点
% 1. 本专利提出了在机器人端到端数据采集过程中引入干扰系统来执行对抗式采集
% 2. 本专利提出了在抓取、转移与放置任务中被操作物体扰动的方法
% 3. 本专利提出了在灵巧操作任务中引入环境破坏方法
% 4. 本专利提出了通过指令干扰，大幅增强机器人端到端神经网络跟随语言指令的能力
% 5. 本专利提出了通过环境障碍物变动，大幅增强机器人端到端神经网络主动避障和精细力控能力



==> 4DWM/Makefile <==
all:
	latexmk --shell-escape --pdf paper.tex

clean:
	rm -f paper.pdf *.aux *.log *.snm *.nav *.fls *.bbl *.blg *.fdb_latexmk *.out *.toc *.brf *.bcf *.run.xml *.idx *.ilg *.ind

main:
	pdflatex paper

full:
	pdflatex paper && \
	bibtex paper && \
	pdflatex paper && \
	pdflatex paper



==> 4DWM/notational_macros.tex <==
\newcommand{\OURS}{\textsc{EnerVerse}\xspace} %
\newcommand{\Ours}{\OURS} %
\newcommand{\OursAudio}{\textsc{Movie Gen Audio}\xspace} %
\newcommand{\OursVideo}{\textsc{Movie Gen Video}\xspace} %
\newcommand{\OursPTV}{\textsc{Personalized Movie Gen Video}\xspace} %
\newcommand{\OursVideoEdit}{\textsc{Movie Gen Edit}\xspace}
\newcommand{\OursVideoEditBench}{Movie Gen Edit Bench\xspace}
\newcommand{\textToVBenchmarkName}{Movie Gen Video Bench\xspace}
\newcommand{\textToVBenchmarkMiniName}{Movie Gen Video Bench-Mini\xspace}
\newcommand{\OursAudioBench}{Movie Gen Audio Bench\xspace}
\newcommand{\OursAudioBenchSGen}{SGen\xspace}
\newcommand{\OursAudioBenchSReal}{SReal\xspace}
\newcommand{\OursAudioBenchMGen}{MGen\xspace}
\newcommand{\CAVTPShort}{CAVTP\xspace}
\newcommand{\IB}{ImageBind\xspace}
\newcommand{\IBShort}{IB\xspace}
\newcommand{\Suno}{External API\xspace}


\newcommand{\TAEone}{\href{https://drive.google.com/file/d/1GacG_e9Y5vx1L7vFQy2IhoshXO63XzRb/view?usp=drive_link}{1}}
\newcommand{\TAEtwo}{\href{https://drive.google.com/file/d/16c4ngm5bQ5qo0XA8AM4yftCYinOrnu57/view?usp=drive_link}{2}}
\newcommand{\TAEthree}{\href{https://drive.google.com/file/d/1phqJme62UAPgKG7xz1_vRJEL6G8Dh2ft/view?usp=drive_link}{3}}

\definecolor{blue300}{HTML}{A4D8FF}

\newcommand{\TextToV}{Text-to-Video\xspace}
\newcommand{\textToV}{text-to-video\xspace}
\newcommand{\imageToV}{image-to-video\xspace}
\newcommand{\imageToVShort}{I2V\xspace}
\newcommand{\ImageToV}{Image-to-Video\xspace}

\newcommand{\textToVShort}{T2V\xspace}
\newcommand{\TextToI}{Text-to-Image\xspace}
\newcommand{\textToI}{text-to-image\xspace}
\newcommand{\videoToA}{video-to-audio\xspace}
\newcommand{\textToIShort}{T2I\xspace}
\newcommand{\textToIVShort}{T2I/V\xspace}
\newcommand{\textImageToVShort}{(T+I)2V\xspace}
\newcommand{\textToImageToVShort}{T2I2V\xspace}
\newcommand{\taeShort}{TAE\xspace}
\newcommand{\tae}{Temporal Autoencoder\xspace}
\newcommand{\upsampler}{Spatial Upsampler\xspace}

\newcommand{\px}{px\xspace}
\newcommand{\flowmatching}{Flow Matching\xspace}
\newcommand{\timeschedule}{t-schedule\xspace}
\newcommand{\llamaNoVersion}{LLaMa\xspace}
\newcommand{\llama}{LLaMa3\xspace}
\newcommand{\llamatwo}{LLaMa2\xspace}
\newcommand{\llamaVideo}{LLaMa3-Video\xspace}
\newcommand{\llamaRewrite}{LLaMa3-FramesRewrite\xspace}

\newcommand{\quality}{Quality\xspace}
\newcommand{\qualityFull}{Visual quality\xspace}
\newcommand{\faithfulness}{Alignment\xspace}
\newcommand{\faithfulnessFull}{Text-alignment\xspace}
\newcommand{\qualityShort}{Q\xspace}
\newcommand{\faithfulnessShort}{A\xspace}
\newcommand{\timestep}{time-step\xspace}
\newcommand{\timesteps}{time-steps\xspace}
\newcommand{\pretraining}{pre-training\xspace}
\newcommand{\pretrained}{pre-trained\xspace}
\newcommand{\Pretraining}{Pre-training\xspace}

\newcommand{\EmuVideo}{Emu-Video\xspace}
\newcommand{\Sora}{OpenAI Sora\xspace}
\newcommand{\LumaLabs}{LumaLabs\xspace}
\newcommand{\Kling}{Kling1.5\xspace}
\newcommand{\RunwayGen}{Runway Gen3\xspace}

\newcommand{\Flux}{Flux.1\xspace}
\newcommand{\Dalle}{OpenAI Dall-E 3\xspace}
\newcommand{\MJ}{Midjourney V6.1\xspace}
\newcommand{\Ideogram}{Ideogram V2\xspace}

\newcommand{\bigO}{$\mathcal{O}$}
\newcommand{\videoDataSize}{\bigO(100)M\xspace} %
\newcommand{\imageDataSize}{\bigO(1)B\xspace}


\newcommand{\viewAsVideoNote}{Figure best viewed in video.\xspace}



\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bx}{\mathbf{X}}
\newcommand{\FMTime}{t}
\newcommand{\FMDiscreteMaxTimeSteps}{N}

\newcommand{\bv}{\mathbf{V}}
\newcommand{\bvin}{\mathbf{V}_\text{in}}
\newcommand{\bvout}{\mathbf{V}_\text{out}}
\newcommand{\bframe}{\mathbf{F}}
\newcommand{\bframeedit}{\mathbf{O}}
\newcommand{\bi}{\mathbf{I}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\vTime}{T'}
\newcommand{\vHeight}{H'}
\newcommand{\vWidth}{W'}
\newcommand{\iTime}{T_{p}}
\newcommand{\timeSmall}{t}
\newcommand{\heightSmall}{h}
\newcommand{\widthSmall}{w}
\newcommand{\bz}{\mathbf{Z}} %
\newcommand{\zTime}{T}
\newcommand{\zHeight}{H}
\newcommand{\zWidth}{W}
\newcommand{\zChannels}{C}
\newcommand{\kTime}{k_{\timeSmall}}
\newcommand{\kHeight}{k_{\heightSmall}}
\newcommand{\kWidth}{k_{\widthSmall}}
\newcommand{\phiTime}{\phi_{\timeSmall}}
\newcommand{\phiHeight}{\phi_{\heightSmall}}
\newcommand{\phiWidth}{\phi_{\widthSmall}}
\newcommand{\prompt}{p} %
\newcommand{\bp}{\mathbf{P}} %
\newcommand{\be}{\mathbf{E}} %
\newcommand{\berev}{\mathbf{E}_\text{rev}}

\newcommand{\videoModel}{f_{v}}



\newcommand{\fixme}[1]{{\color{red} \textbf{#1}}}




\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}


\newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.33\textheight][c]{0.5\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


==> abstract.tex <==
\abstract{


}

